Strong-Lensing Analysis of MACS,J0717.5+3745 from Hubble Frontier Fields observations: How well can the mass distribution be constrained?

[abridged] We present a strong-lensing analysis of MACSJ0717.5+3745, based on the full depth of the Hubble Frontier Field (HFF) observations, which brings the number of multiply imaged systems to 61, ten of which are spectroscopically confirmed. The total number of images comprised in these systems rises to 165. Our analysis uses a parametric mass reconstruction technique, as implemented in the Lenstool software, to constrain a mass distribution composed of four large-scale mass components + galaxy-scale perturbers. We find a superposition of cored isothermal mass components to provide a good fit to the observational constraints, resulting in a very shallow mass distribution for the smooth (large-scale) component. Given the implications of such a flat mass profile, we investigate whether a model composed of "peaky" non-cored mass components can also reproduce the observational constraints. We find that such a non-cored mass model reproduces the observational constraints equally well. Although the total mass distributions of both models are consistent, as well as the integrated two dimensional mass profiles, we find that the smooth and the galaxy-scale components are very different. We conclude that, even in the HFF era, the generic degeneracy between smooth and galaxy-scale components is not broken, in particular in such a complex galaxy cluster. Consequently, insights into the mass distribution of MACS J0717 remain limited, underlining the need for additional probes beyond strong lensing. Our findings also have implications for estimates of the lensing magnification: we show that the amplification difference between the two models is larger than the error associated with either model. This uncertainty decreases the area of the image plane where we can reliably study the high-redshift Universe by 50 to 70%.

==> magtable.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{ccccc}
\hline
ID & Ampli (cored) & Ampli (non-cored) & $\Delta$ [cored\,-\,noncored] & $\Delta$ [pre-HFF]  \\
\hline \\*[-1mm]
19.3 & 3.2 $\pm$0.15 [21]  & 2.8$\pm$0.07 [40] & 0.4  & 1.7  \\
68.2 & 24$\pm$2.0 [12] & 8.7$\pm$0.6 [14.5]  & 15.3  & 4.0  \\
71.2 & 12.0$\pm$1.4 [8.5] & 10.0$\pm$0.7 [14] & 2.0 & 63.5 \\ 
61.2 &  2.3$\pm$0.2 [11.5] & 1.6$\pm$0.1 [16] & 0.7 & 1.62 \\
57.1 & 12.3$\pm$6.0 [2] & 32.4$\pm$ 846 [$<$1] & $>100$ & 205 \\
23.2 & 1083$\pm$9167 [$<$1] & 21.8$\pm$2.5 [$<1$] & $>1000$ & 69 \\
\hline
\smallskip
\end{tabular}
\end{center}
\caption{
For different multiple images, we report: the value of the amplification with associated errors
and signal to noise ratio (into brackets), for the cored and the non-cored model; the difference in amplification between the cored and the
non-cored mass model; the difference in amplification considering pre-HFF data and the different
modeling/group software. Magnifications computed for $z=3.0$.}
\label{magtable}
\end{table*}


==> table.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{cccccc}
\hline
ID & R.A. & Decl. & $z_{\rm spec}$ & $z_{\rm model}$ (\emph{non-cored}, \emph{cored}, NFW) & $z_{\rm phot}$\\
\hline \\*[-1mm]
%1.1$^{*}$ & 109.39587 & 37.74212 & 2.963 & -- \\ %strong Ly_alpha
1.1 & 109.39534 & 37.741178 & -- & --  & 3.07$\pm$0.06\\
1.2 & 109.39382 & 37.740095 & 2.963 & -- & 2.91$\pm$0.09\\
1.3 & 109.39098 & 37.738280 & 2.963 & -- &2.72$\pm$0.17\\
1.4 & 109.38436 & 37.736945 & --  & -- &3.11$\pm$0.06\\
1.5 & 109.40578 & 37.761378 & --  & -- &3.11$\pm$0.07\\
2.1 & 109.39281 & 37.741010 & --  & 2.6$\pm$0.3, 2.2$\pm$0.4, 3.0$\pm$0.3 &2.72$\pm$0.12\\ 
2.2 & 109.39043 & 37.739245 & --  & -- &2.72$\pm$0.07 \\ 
3.1 & 109.39855 & 37.741495 & 1.855  & -- & 1.87$\pm$0.04\\
3.2 & 109.39446 & 37.739176 & 1.855 & -- & 1.84$\pm$0.04\\
3.3 & 109.40715 & 37.753827 & 1.855  & -- & 1.84$\pm$0.04\\
4.1 & 109.38088 & 37.750127 & 1.855 & -- & 1.93$\pm$0.05\\
4.2 & 109.37644 & 37.744696 & 1.855  & --  & 1.84$\pm$0.04\\
4.3 & 109.39109 & 37.763296 & 1.855  & --  &1.82$\pm$0.04\\
5.1 & 109.37991 & 37.746861 & --  & 4.1$\pm$0.2, 3.8$\pm$0.2, 3.7$\pm$0.1  & --\\
5.2 & 109.37791 & 37.742810 & --  & -- &--\\
5.3 & 109.40003 & 37.767399 & --  & -- &--\\
6.1 & 109.36436 & 37.757091 & 2.393  & -- &2.37$\pm$0.06\\
6.2 & 109.36271 & 37.752693 & 2.393  & -- &2.27$\pm$0.07\\
6.3 & 109.37388 & 37.769711 & 2.393  & -- & --\\
7.1 & 109.36657 & 37.766343 & --  & 1.9$\pm$0.1, 2.0$\pm$0.1, 2.0$\pm$0.1 & -- \\
7.2 & 109.36505 & 37.764125 & --  & --& --\\
7.3 & 109.35905 & 37.751780 & --  & -- & 2.23$\pm$0.13\\  
8.1 & 109.36665 & 37.769694 & --  & 2.5$\pm$0.1, 2.9$\pm$0.2, 2.8$\pm$0.1 &--\\
8.2 & 109.36208 & 37.763125 & --  & -- &--\\
8.3 & 109.35652 & 37.751928 & --  & -- &--\\
12.1 &109.38516 & 37.751844 & 1.699  & -- &1.62$\pm$0.05 \\
12.2 &109.37762 & 37.742878 & 1.699  & -- &1.73$\pm$0.06\\
12.3 &109.39122 & 37.760626 & 1.699  & -- &1.71$\pm$0.05\\
13.1 &109.38567 & 37.750733 &2.547& -- & 2.47$\pm$0.06\\ 
13.2 &109.37756 & 37.739627 & --  & -- &2.54$\pm$0.07\\
13.3 &109.39621 & 37.763333 & 2.540  & -- &2.61$\pm$0.09\\
14.1 &109.38879 & 37.752163 & 1.855  & -- &1.84$\pm$0.04\\
14.2 &109.37966 & 37.739707 & 1.855  & -- &1.84$\pm$0.04\\
14.3 &109.39619 & 37.760427 & 1.855  & --  &1.84$\pm$0.02\\
15.1 &109.36766 & 37.772059 & 2.405 & -- & --\\
15.2 &109.35862 & 37.760127 & --  & --  &--\\
15.3 &109.35654 & 37.754641 & --  & --  & 3.40$\pm$0.08\\
16.1 &109.36916 & 37.773279 & --  & 3.2$\pm$0.3, 3.6$\pm$0.3, 3.1$\pm$0.1 &-- \\
16.2 &109.35856 & 37.759558 & --  & --  &--\\
16.3 &109.35694 & 37.753691 & --  & --  &--\\
17.1 &109.36938 & 37.771869 & --  & 2.7$\pm$0.2, 2.8$\pm$0.2, 2.7$\pm$0.1 &-- \\
17.2 &109.35938 & 37.758792 & --  & --  &--\\
17.3 &109.35822 & 37.753609 & --  & --  & 3.15$\pm$0.14\\
18.1 &109.36425 & 37.768628 & --  & 2.0$\pm$0.1, 2.6$\pm$0.5, 2.2$\pm$0.1 &-- \\
18.2 &109.36121 & 37.764326 & --  & --  &-- \\
19.1 &109.40906 & 37.754681 & 6.40 & -- &-- \\
19.2 &109.40772 & 37.742731 & 6.40 & -- &-- \\
19.3 &109.38105 & 37.731391 & 6.40 & -- &-- \\
\hline
\smallskip
\end{tabular}
\end{center}
\caption{Multiple-image systems found before the FF observations.
Uncertainties quoted for redshifts predicted by our model, $z_{\rm model}$,  correspond to the 1$\sigma$ 
confidence level. They are given for the \emph{non-cored}, the \emph{cored}, and the NFW models.
In the last column, we show the estimate of the photometric redshift, when possible, together
with the 1$\sigma$ error bars.}
\label{multipletable1}
\end{table*}


==> table2.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{cccccc}
\hline
ID & R.A. & Decl. & $z_{\rm spec}$ & $z_{\rm model}$ (\emph{non-cored}, \emph{cored}, NFW) & $z_{\rm phot}$\\
\hline \\*[-1mm]
20.1 & 109.37420 & 37.7651450 & -- & 3.4$\pm$1.0, $>$2.6, uncons. &-- \\
20.2 & 109.37340 & 37.7646610 & -- & -- &-- \\
21.1* & 109.37241 & 37.746392 & -- & -- &2.61$\pm$0.16\\
21.2* & 109.37673 & 37.752029 & -- & -- & 2.65$\pm$0.12\\
22.1* & 109.36773 & 37.755897 & -- & -- & 0.87$\pm$0.11\\
22.2* & 109.36769 & 37.755556 & -- & -- & 0.93$\pm$0.05\\
23.1* & 109.37958 & 37.762879 & -- & -- & --\\
23.2* & 109.37897 & 37.761983 & -- & -- &-- \\
24.1 & 109.392290 & 37.732946 & -- & 2.7$\pm$0.1, 2.5$\pm$0.1, 2.5$\pm$0.1 &--\\
24.2 & 109.410560 & 37.748427 & -- & -- &--\\
25.1 & 109.380290 & 37.744746 & -- & 4.0$\pm$0.1, 3.8$\pm$0.1, 3.8$\pm$0.2 &--\\
25.2 & 109.379510 & 37.742762 & -- & -- &--\\
25.3 & 109.402910 & 37.766411 & -- & -- &--\\
27.1 & 109.397390 & 37.747883 & -- & 1.6$\pm$0.9, 3.0$\pm$1.1, uncons. & 2.95$\pm$0.18\\
27.2 & 109.397560 & 37.747567 & -- & -- & 2.17$\pm$0.32\\
29.1 & 109.400870 & 37.743174 & -- & 1.7$\pm$0.1, 1.7$\pm$0.1, 1.7$\pm$0.1 & 1.45$\pm$0.07\\
29.2 & 109.392840 & 37.738612 & -- & -- &1.62$\pm$0.06\\
31.1 & 109.374720 & 37.756347 & -- & 1.6$\pm$0.1, 1.6$\pm$0.1, 1.6$\pm$0.1 &1.55$\pm$0.08\\
31.2 & 109.371000 & 37.750538 & -- & -- &1.52$\pm$0.06\\
31.3 & 109.381610 & 37.764973 & -- & -- &1.57$\pm$0.08\\
32.1 & 109.369500 & 37.757729 & -- & 2.3$\pm$0.1, 2.8$\pm$0.1, 2.5$\pm$0.1 & --\\
32.2 & 109.380950 & 37.769382 & -- & -- & --\\
32.3 & 109.366250 & 37.749210 & -- & -- & 2.40$\pm$0.05\\
33.1 & 109.383770 & 37.758259 & -- & 3.5$\pm$0.3, 3.7$\pm$0.2, 3.7$\pm$0.1 &--\\
33.2 & 109.386620 & 37.764144 & -- & -- &--\\
33.3 & 109.370370 & 37.738712 & -- & -- &--\\
34.1 & 109.391580 & 37.766308 & -- & 2.6$\pm$0.2, 2.7$\pm$0.2, 2.6$\pm$0.1 &--\\
34.2 & 109.379110 & 37.751227 & -- & -- &1.03$\pm$0.05\\
34.3 & 109.373300 & 37.744211 & -- & -- &1.11$\pm$0.09\\
36.1 & 109.364330 & 37.771976 & -- &2.4$\pm$0.2, 2.9$\pm$0.2, 2.6$\pm$0.1 &--  \\
36.2 & 109.358240 & 37.763325 & -- & -- &--\\
36.3 & 109.353290 & 37.755808 & -- & -- &--\\
37.1 & 109.397090 & 37.754736 & -- & 3.8$\pm$0.8, 3.3$\pm$0.7, 3.3$\pm$0.4 &--\\
37.2 & 109.396720 & 37.754793 & -- & -- &--\\
39.1 & 109.402270 & 37.731234 & -- & 4.3$\pm$0.3, 4.1$\pm$0.3, 4.1$\pm$0.3 &1.82$\pm$0.04\\
39.2 & 109.404950 & 37.732519 & -- & -- & 2.14$\pm$0.19\\
39.3* & 109.414740 & 37.743276 & -- & -- &--\\
45.1 & 109.389820 & 37.739214 & -- & 2.7$\pm$0.1, 2.7$\pm$0.1, 2.6$\pm$0.1 &--\\
45.2 & 109.383480 & 37.737879 & -- & -- &--\\
45.3 & 109.404470 & 37.761960 & -- & -- &-- \\
49.1 & 109.402800 & 37.733260 & -- & $>$4.8, 4.1$\pm$0.3, 3.8$\pm$0.2 & 3.40$\pm$0.08\\
49.2 & 109.393000 & 37.730812 & -- & -- & 3.54$\pm$0.06\\
50.1 & 109.374440 & 37.743736 & -- & 3.7$\pm$0.4, 3.6$\pm$0.3, 3.6$\pm$0.2 & 3.19$\pm$0.10\\
50.2 & 109.379580 & 37.750708 & -- & -- &--\\
50.3* & 109.392800 & 37.767181 & -- & -- &--\\
52.1 & 109.368380 & 37.771761 & -- & 3.0$\pm$0.2, 3.3$\pm$0.2, 3.3$\pm$0.3 &--\\
52.2 & 109.360230 & 37.760497 & -- & -- &--\\
52.3 & 109.357040 & 37.752486 & -- & -- &--\\
55.1 & 109.373760 & 37.755778 & -- & 2.2$\pm$0.1, 2.4$\pm$0.1, 2.4$\pm$0.1 & --\\
55.2 & 109.370240 & 37.748743 & -- & -- & 2.17$\pm$0.11\\
55.3 & 109.385020 & 37.768411 & -- & -- & --\\
56.1 & 109.373150 & 37.744015 & -- & 3.2$\pm$0.2, 3.2$\pm$0.2, 3.0$\pm$0.1 &--\\
56.2 & 109.378400 & 37.751095 & -- & -- &--\\
56.3* & 109.391820 & 37.766216 & -- & -- &--\\
57.1 & 109.379030 & 37.744097 & -- & 1.7$\pm$0.1, 1.8$\pm$0.2, 1.7$\pm$0.1 &--\\
57.2 & 109.379530 & 37.745110 & -- & -- &--\\
58.1 & 109.379420 & 37.762383 & -- & 4.2$\pm$1.4, 4.2$\pm$1.2, uncons. &3.03$\pm$0.34 \\
58.2 & 109.379260 & 37.762129 & -- & -- & --\\
59.1 & 109.376840 & 37.743245 & -- & 3.4$\pm$0.8, 4.2$\pm$0.5, 3.6$\pm$0.5 &3.11$\pm$0.23\\
59.2 & 109.379960 & 37.748146 & -- & -- &--\\
59.3* & 109.400700 & 37.768628 & -- & -- &--\\
62.1 & 109.372220 & 37.747464 & -- & 2.7$\pm$0.3, 2.9$\pm$0.3, 2.7$\pm$0.3 &2.23$\pm$0.08 \\
62.2 & 109.375510 & 37.752276 & -- & -- & 2.23$\pm$0.06\\ 
63.1 & 109.369420 & 37.756278 & -- & 1.3$\pm$0.1, 1.6$\pm$0.1, 1.7$\pm$0.1 & 2.20$\pm$0.24\\
63.2 & 109.368360 & 37.753695 & -- & -- & 2.20$\pm$0.18\\ 
64.1* & 109.372250 & 37.765391 & -- & -- &--\\
64.2* & 109.371790 & 37.765066 & -- & -- &--\\
\hline
\smallskip
\end{tabular}
\end{center}\caption{Multiple-image systems found after the FF observations.
Images with * are the ones we propose as candidates and that are not used as
constraints in the mass model.
Uncertainties quoted for redshifts predicted by our model, $z_{\rm model}$,  correspond to the 1$\sigma$
confidence level. They are given for the \emph{non-cored}, the \emph{cored}, and the NFW model.
uncons means unconstrained, \emph{i.e.} when the output PDF is flat.
In the last column, we show the estimate of the photometric redshift, when possible, together
with the 1$\sigma$ error bars.
}
\label{multipletable2}
\end{table*}



\begin{table*}
\begin{center}
\begin{tabular}{cccccc}
\hline
ID & R.A. & Decl. & $z_{\rm spec}$ & $z_{\rm model}$ (\emph{non-cored}, \emph{cored}, NFW) & $z_{\rm phot}$\\
\hline \\*[-1mm]

65.1 & 109.383120 & 37.762595 & -- & 5.4$\pm$0.3, $>$4.6, $>$5.0 & --\\
65.2 & 109.382250 & 37.760394 & -- & -- & -- \\
66.1 & 109.383310 & 37.765079 & -- & $>$6.5, 6.4$\pm$0.8, 6.5$\pm$0.4 & --\\
66.2 & 109.380290 & 37.759228 & -- & -- & --\\
67.1 & 109.367470 & 37.756509 & -- & 3.0$\pm$0.1, 4.2$\pm$0.9, 4.5$\pm$0.5 & --\\
67.2 & 109.365120 & 37.749544 & -- & -- & --\\
67.3* & 109.382090 & 37.771629 & -- & -- & --\\
68.1 & 109.392330 & 37.738083 & 5.51 & -- & --\\
68.2 & 109.382350 & 37.736508 & -- & -- & --\\
68.3* & 109.406780 & 37.763803 & -- & -- & --\\
69.1 & 109.380400 & 37.749467 & -- & 3.4$\pm$0.5, 3.3$\pm$0.4, 3.1$\pm$0.4 & --\\
69.2 & 109.375320 & 37.743383 & -- & -- & --\\
69.3* & 109.396440 & 37.768591 & -- & -- & --\\
70.1 & 109.392210 & 37.760496 & -- & 3.7$\pm$0.4, 3.1$\pm$0.2, 3.9$\pm$0.3 & 2.72$\pm$0.06\\
70.2 & 109.389380 & 37.757279 & -- & -- &3.11$\pm$0.07\\
70.3* & 109.375110 & 37.735945 & -- & -- &2.14$\pm$0.09\\
71.1 & 109.382700 & 37.744711 & -- & 3.0$\pm$0.1, 2.6$\pm$0.1, 2.6$\pm$0.1 &2.91$\pm$0.10\\
71.2 & 109.380650 & 37.741346 & -- & -- &1.82$\pm$0.04\\
71.3 & 109.402550 & 37.763610 & -- & -- &2.65$\pm$0.16\\
71.4 & 109.387210 & 37.741295 & -- & -- & -- \\
72.1 & 109.380120 & 37.765496 & -- & $>$4.1, $>$4.0, 3.9$\pm$0.4 &3.32$\pm$0.14\\
72.2 & 109.374810 & 37.762346 & -- & -- &3.32$\pm$0.22\\
73.1* & 109.375970 & 37.748883 & -- & -- &--\\
73.2* & 109.375500 & 37.748483  & -- & -- &--\\
73.3* & 109.391470 & 37.767033  & -- & -- &--\\
74.1* & 109.370890 & 37.751182  & -- & -- & 1.52$\pm$0.06\\
74.2* & 109.383420 & 37.769708  & -- & -- &--\\
74.3* & 109.371310 & 37.751974  & -- & -- &1.60$\pm$0.15\\
75.1 & 109.382000 & 37.738429  & -- & 3.6$\pm$0.4, 4.7$\pm$0.4, 4.3$\pm$0.5  &--\\
75.2 & 109.388640 & 37.739263  & -- & -- &--\\
75.3* & 109.40496 & 37.764678  & -- & -- &--\\
76.1 & 109.411230 & 37.731990  & -- & 4.5$\pm$0.4, 5.4$\pm$0.3,3.7$\pm$0.4 &--\\
76.2 & 109.412840 & 37.733789 & -- & -- &--\\
76.3 & 109.413660 & 37.734646 & -- & -- &--\\
77.1* & 109.377000 & 37.736456 & -- & -- &--\\
77.2* & 109.386260 & 37.751928 & -- & -- &--\\
77.3* & 109.399110 & 37.764959 & -- & -- &--\\
78.1* & 109.371840 & 37.742478 & -- & -- &--\\
78.2* & 109.379010 & 37.752778 & -- & -- &--\\
79.1 & 109.393150 & 37.762795  & -- & 3.7$\pm$0.3, 3.4$\pm$0.2,3.7$\pm$0.3 &--\\
79.2 & 109.387350 & 37.755963 & -- & -- &--\\
79.3 & 109.375740 & 37.735628 & -- & -- &--\\
80.1 & 109.390940 & 37.733628 & -- & 3.7$\pm$0.3, 3.3$\pm$0.1, 3.8$\pm$0.2 & 2.37$\pm$0.15 \\
80.2 & 109.400250 & 37.738496 & -- & -- & 2.50$\pm$0.11 \\
80.3 & 109.410080 & 37.753576 & -- & -- & 2.40$\pm$0.14 \\
81.1* & 109.408320 & 37.728127  & -- & -- & --  \\
81.2* & 109.409010 & 37.728544  & -- & -- & -- \\
81.3* & 109.410160 & 37.729344 & -- & -- & -- \\
82.1* & 109.383660 & 37.766146 & -- & -- & 2.65$\pm$0.48 \\
82.2* & 109.379500 & 37.756303 & -- & -- & 2.72$\pm$0.21 \\
\hline
\smallskip
\end{tabular}
\end{center}
\caption{... continued ... }
\label{multipletable2}
\end{table*}


==> tableres.tex <==
\begin{table*}
\begin{center}
\begin{tabular}[h!]{cccccccc}
\hline
\hline
\noalign{\smallskip}
Component  & $\Delta$ \textsc{ra}  & $\Delta$ \textsc{dec} & $e$ & $\theta$ & r$_{\mathrm{core}}$ (\arcsec) &  r$_{\mathrm{s}}$ (\arcsec)   &$\sigma$ (\footnotesize{km\,s$^{-1}$})\\ 
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\noalign{\smallskip}
C &  -9.1$^{+1.5}_{-0.5}$  & -8.7 $\pm$ 1.4  &  0.34 $\pm$ 0.03 &  54 $\pm$ 4 &  16.1 $\pm$ 2.0 & [1000] & 895 $\pm$ 29.0 \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
D &  26.6 $\pm$ 0.9  & -19.3 $\pm$ 1.1 & 0.65 $\pm$ 0.03 &  52 $\pm$ 3  &  4.5 $\pm$ 0.8  & [1000] & 494$\pm$15  \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
B &  37.3 $\pm$ 3.9  & 34.9 $\pm$ 1.8  &  0.50 $\pm$ 0.06  &  3$^{+9}_{-2}$  &  27.6 $\pm$ 2.1 & [1000] & 800 $\pm$ 38 \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
A &  114.9 $\pm$ 2.9  & 64.7 $\pm$ 1.1  & 0.68 $\pm$ 0.01 &  9 $\pm$ 5  &  20.7 $\pm$ 2.1  & [1000]  & 880 $\pm$ 22  \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
L$^*$ galaxy & --  & --  & --    &    --   &  [0.05] &  8.3 $\pm$ 0.7  & 250.3 $\pm$ 8.4 \\
\noalign{\smallskip}
\hline
\hline
\end{tabular}
\caption{dPIE parameters inferred for the dark matter components considered in the optimization procedure: the four large scale dark matter clumps (A, B, C, D)
and the galaxy scale component. These parameters correspond to the \emph{cored} mass model.
Coordinates are given in arcseconds with respect to
$\alpha=109.3982, \delta=37.745778$.
The ellipticity $e$ is the one of the mass distribution.
Error bars correspond to $1\sigma$ confidence level.
Parameters in brackets are not optimized.
Concerning the scaling relations, the zero point is set
to a magnitude equal to 20.66.
}
\label{tableres}
\end{center}
\end{table*}


==> tableres2.tex <==
\begin{table*}
\begin{center}
\begin{tabular}[h!]{cccccccc}
\hline
\hline
\noalign{\smallskip}
Component  & $\Delta$ \textsc{ra}  & $\Delta$ \textsc{dec} & $e$ & $\theta$ & r$_{\mathrm{core}}$ (\arcsec) &  r$_{\mathrm{s}}$ (\arcsec)   &$\sigma$ (\footnotesize{km\,s$^{-1}$})\\ 
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\noalign{\smallskip}
C &  -0.9 $\pm$ 0.5  & 4.9$^{+0.1}_{-0.5}$  &  $>$ 0.38 &  63 $\pm$ 2 & 4.9$^{+0.1}_{-0.2}$ & [1000] & 889 $\pm$ 11  \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
D &  31.8 $\pm$ 0.5 & -14.5 $\pm$ 0.5 & $>$ 0.69 & 46 $\pm$ 3 &  4.8 $\pm$ 0.2  & [1000] & 617 $\pm$ 8  \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
B &  64.9 $\pm$ 1.0  & 39.9$^{+0.1}_{-0.2}$  &  $>$ 0.54  &  173 $\pm$ 18 &  4.9$^{+0.1}_{-0.6}$ & [1000] & 733 $\pm$ 13 \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
A &  134.9$^{+0.1}_{-0.7}$  & 75.0$^{+0.5}_{-0.1}$  & 0.61 $\pm$ 0.03 &  12.0 $\pm$ 9  &  2.7 $\pm$ 0.4  & [1000]  & 795 $\pm$ 16  \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
L$^*$ galaxy & --  & --  & --    &    --   &  [0.05] &  11.4 $\pm$ 1.4  & 161 $\pm$ 6\\
\noalign{\smallskip}
\hline
\hline
\end{tabular}
\caption{Same as Table~\ref{tableres}, for the \emph{non-cored} mass model.
}
\label{tableres2}
\end{center}
\end{table*}



==> tableres3.tex <==
\begin{table*}
\begin{center}
\begin{tabular}[h!]{cccccccc}
\hline
\hline
\noalign{\smallskip}
Component  & $\Delta$ \textsc{ra}  & $\Delta$ \textsc{dec} & $e$ & $\theta$ & c$_{\mathrm{200}}$ &  r$_{\mathrm{s}}$ (\arcsec)   &$\sigma$ (\footnotesize{km\,s$^{-1}$})\\ 
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\noalign{\smallskip}
C &  -2.3 $\pm$ 0.6 & -0.7 $\pm$ 0.8  &  0.13 $\pm$ 0.02 &  53 $\pm$ 4 &  3.4 $\pm$ 0.2 & 81.8 $\pm$ 6.0 & -- \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
D &  32.6 $\pm$ 0.4  & -13.5 $\pm$ 0.5 & 0.55 $\pm$ 0.03 &  50 $\pm$ 2  &  5.3 $\pm$ 0.3  & 25.3 $\pm$ 2.2 & --  \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
B &  63.3 $\pm$ 1.2  & 44.6 $\pm$ 0.4  &  0.51 $\pm$ 0.06  &  5 $\pm$ 2  & 3.0$^{+0.1}_{-0.0}$ & 63.9 $\pm$ 3.7 & -- \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
A &  133.7 $\pm$ 0.9  & 77.4 $\pm$ 1.4  & 0.23 $\pm$ 0.04 &  165 $\pm$ 15  &  5.5 $\pm$ 0.3  & 32.5 $\pm$ 0.35  & --  \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
L$^*$ galaxy & --  & --  & --    &    --   &  -- &  9.2 $\pm$ 0.4  & 188 $\pm$ 9 \\
\noalign{\smallskip}
\hline
\hline
\end{tabular}
\caption{NFW parameters inferred for the four large scale dark matter clumps (A, B, C, D), and dPIE parameters for
the galaxy scale component (the core radius being fixed to 0.3\,kpc). These parameters correspond to the NFW mass model.
Coordinates are given in arcseconds with respect to
$\alpha=109.3982, \delta=37.745778$.
The ellipticity $e$ is the one of the mass distribution.
Error bars correspond to $1\sigma$ confidence level.
Concerning the scaling relations, the zero point is set
to a magnitude equal to 20.66.
}
\label{tableres3}
\end{center}
\end{table*}

